Shock-Shock Interaction in the Jet of CTA 102

The radio light curve and spectral evolution of the blazar CTA 102 during its 2006 outburst can be rather well explained by the standard shock-in-jet model. The results of a pixel-to-pixel spectral analysis of multi-frequency VLBI images, together with kinematics derived from the MOJAVE survey lead to the picture of an over-pressured jet with respect to the ambient medium. The interaction of a traveling shock wave with a standing one is a possible scenario which could explain the observed spectral behaviour

==> pagen.tex <==
{97}

